A Taxonomy and Methodology for Proof-of-Location Systems

Digital societies increasingly rely on trustworthy proofs of physical presence for services such as supply-chain tracking, e-voting, ride-sharing, and location-based rewards. Yet, traditional localization methods often lack cryptographic guarantees of where and when an entity was present, leaving them vulnerable to spoofing, replay, or collusion attacks. In response, research on Proof-of-Location (PoL) has emerged, with recent approaches combining distance bounding, distributed consensus, and privacy-enhancing techniques to enable verifiable, tamper-resistant location claims. As the design space for PoL systems grows in complexity, this paper provides a unified framework to help practitioners navigate diverse application needs. We first propose a taxonomy identifying four core domains: (1) cryptographic guarantees, (2) spatio-temporal synchronization, (3) trust and witness models, and (4) interaction and overhead. Building on this, we introduce a methodology to map application-specific requirements onto appropriate PoL architectures. We illustrate this process through three use cases (retail e-coupons, supply chain auditing, and physical e-voting), each showing how different constraints shape protocol choices. Overall, this work offers a structured approach to building secure, scalable, and interoperable PoL systems.

==> sections/06-logic.tex <==
Recent advances in \pol{} systems have generated diverse protocols, each using a 
combination of distance bounding, timestamps, and consensus-based verification. 
Amidst this growing variety, there is a need to standardize how we express 
location claims and to build a unified theoretical foundation for \pol{}. 
This section provides a first attempt at formally capturing 
``Prover $p$ was in region $\ell$ at time $t$'' in a spatiotemporal logic, 
highlighting how completeness and soundness map onto these claims. 
By anchoring \pol{} protocols in a consistent formal language, 
we can better compare, compose, and eventually standardize location-proof designs.

\subsection{Basic Definitions and Notation}
\label{sec:logic-basics}

Let $\mathcal{P}$ be the set of potential \emph{provers} (e.g., users or devices), 
and let $\mathcal{L}$ be the set of \emph{locations}, which may range from 
fine-grained coordinates to coarse zones (Section~\ref{sec:taxonomy-spacetime}). 
We define:
\[
\mathrm{Loc}(p, \ell, t) \quad\text{as the statement ``Prover $p$ is in location $\ell$ at time $t$.''}
\]
Here, $t$ may be a discrete block index or a timestamp from a continuous timeline. 
In some contexts, we consider intervals, $\mathrm{Loc}(p, \ell, [t_1, t_2])$, 
to represent sustained presence over a duration.

\subsection{Spatiotemporal Formulas}
\label{sec:logic-formulas}

Location claims often require more detail, such as distance constraints 
or the ordering of events:
\begin{itemize}
    \item \emph{Proximity constraints}: 
    $\mathrm{Dist}(p,a) \le d \;\Rightarrow\; \mathrm{Loc}(p,\ell,t)$, 
    where anchor $a$ is known to lie within region $\ell$. 
    This encodes \emph{proximity soundness} (\S\ref{sec:taxonomy-crypto}).

    \item \emph{Temporal ordering}: 
    $\mathrm{Time}(b_i) < \mathrm{Time}(b_{i+1})$, indicating 
    an event in block $b_i$ precedes one in $b_{i+1}$. 
    This matches how ledgers or PBFT-style consensus define a 
    global sequence of proofs (\S\ref{sec:taxonomy-spacetime}).
\end{itemize}
Such formulas enable \emph{distance bounding} (``$p$ is within $d$ meters of anchor $a$'') 
and event ordering (``this proof must come before block $b_{i+1}$''), 
elements seen in high-precision or real-time scenarios 
like e-voting (\S\ref{sec:usecases-evoting}).

\subsection{Completeness and Soundness}
\label{sec:logic-completeness-soundness}

\paragraph{Completeness.}
A \pol{} protocol is \emph{complete} if, whenever $\mathrm{Loc}(p,\ell,t)$ 
is \emph{actually} true, the protocol’s verification accepts that claim 
with overwhelming probability:
\[
   \mathrm{Pr}\Bigl[\text{ProtocolAccept} \;\mid\; \mathrm{Loc}(p,\ell,t)\Bigr] \approx 1.
\]

\paragraph{Soundness.}
Likewise, it is \emph{sound} if, whenever $\mathrm{Loc}(p,\ell,t)$ 
is \emph{false}, any attempted proof fails with high probability:
\[
   \mathrm{Pr}\Bigl[\text{ProtocolAccept} \;\mid\; \neg\, \mathrm{Loc}(p,\ell,t)\Bigr] \approx 0.
\]
For \pol{} systems, we refine $\mathrm{Loc}$ to incorporate 
\emph{Proximity Soundness} (distance bounding) and 
\emph{Temporal Soundness} (secure timestamps), ensuring $p$ cannot lie 
about \emph{where} or \emph{when} it was.

\subsection{Interpreting Cryptographic Proofs in Logic}
\label{sec:logic-proof-interpretation}

Each valid proof output by a protocol can be viewed as evidence for a formula, e.g.,
\[
  \mathrm{Loc}(p,\ell,t) \;\wedge\; \mathrm{TimeSync}(\ell, t),
\]
where $\mathrm{TimeSync}(\ell,t)$ indicates that the proof includes 
a consensus-based or anchor-based timestamp consistent with $t$. 
Distance-bounding transcripts or zero-knowledge statements further refine 
$\mathrm{Loc}(p,\ell,t)$, encoding that ``$p$ is \emph{actually} within bounding distance $d$ 
of anchor(s) in $\ell$,'' which relates closely to the multi-witness 
triangulation used in the \emph{E-Voting} scenario (\S\ref{sec:usecases-evoting}) 
or the partial distribution used in \emph{Supply Chain Auditing} (\S\ref{sec:usecases-supplychain}).

\subsection{Example: Single Anchor vs.\ Multi-Witness}
\label{sec:logic-examples}

\paragraph{Single Anchor.}
If $p$ obtains a signature $\sigma = \mathrm{Sign}_A(p,\ell,t,\dots)$ 
from a trusted anchor $A$, we interpret $\sigma$ as 
\[
  \mathrm{Loc}(p,\ell,t) \;\;\leftarrow\;\; \mathrm{TrustedAnchor}(A).
\]
In simpler scenarios like the \emph{Retail E-Coupon} case (\S\ref{sec:usecases-retail}), 
this alone may suffice, albeit with weaker collusion resistance.

\paragraph{Multi-Witness Triangulation.}
In a decentralized scenario with $W_1,\dots,W_n$ (e.g.\ E-Voting or partial distribution 
in supply chains), each partial signature or ephemeral time-of-flight measure 
collectively implies
\[
 \mathrm{Loc}(p,\ell,t) \quad\iff\quad \bigwedge_{i=1}^{n}\,\mathrm{Dist}(p,W_i) \le d_i,
\]
assuming the protocol ensures consensus on time $t$. 
This higher complexity aligns with the methodology’s recommendation 
for high-stakes or fine-grained scenarios.

\subsection{Toward a Unified Theory of Location Proofs}
\label{sec:logic-discussion}

By formalizing \pol{} claims as logical formulas, we unify diverse protocols under 
a single conceptual lens, clarifying how \emph{completeness} and \emph{soundness} 
translate into spatiotemporal correctness. This shared framework allows:

\begin{itemize}
    \item \textbf{Comparability}: We can assess whether two protocols 
    achieve the same level of distance bounding or time integrity, 
    using the same logical statements and definitions.
    \item \textbf{Modularity}: New constructs (e.g.\ zero-knowledge or threshold signatures) 
    can be added to the logic as sub-formulas (``$\mathrm{ZK}(p,\ell)$'') 
    that preserve completeness/soundness under composition.
    \item \textbf{Standardization Efforts}: As \pol{} technology evolves (see, e.g., 
    \cite{foam-white-paper} on decentralized mapping), formal semantics help the community 
    converge on consistent definitions, bridging academic protocols and industry standards.
\end{itemize}

\paragraph{Connection to the Use Cases.}
In Sections~\ref{sec:usecases-retail}--\ref{sec:usecases-supplychain}, 
we illustrated how different demands on precision, threat level, and trust model 
produce distinct architectural choices. Each resulting solution can be seen 
as implementing a \emph{logical rule} that validates $\mathrm{Loc}(p,\ell,t)$ 
with varying degrees of strictness:
\begin{itemize}
  \item The \emph{Retail E-Coupon} case effectively states 
  ``One anchor’s signature $\sigma$ implies $\mathrm{Loc}(p,\ell,t)$ 
  for coarse $\ell$ and day-level $t$.''

  \item The \emph{E-Voting} scenario encodes 
  ``$\bigwedge_{i=1}^{n}\mathrm{Dist}(p,W_i)\le d_i \,\wedge\,
    \mathrm{BlockOrder}(t)$ $\implies$ $\mathrm{Loc}(p,\ell,t)$,'' 
  capturing sub-meter bounding, multi-witness, and a timestamp ledger 
  to verify presence in the correct window.

  \item The \emph{Supply Chain} approach uses partial distribution 
  with looser distance constraints, etc.
\end{itemize}

\noindent
Such a logical view fosters a more rigorous approach to \pol{} protocol design, 
highlighting exactly which premises must hold to ensure the final statement 
(``$p$ was in $\ell$ at $t$'') is \emph{sound}.

While this formalization demonstrates how spatiotemporal proofs map onto 
completeness/soundness criteria, much remains to be done to create 
a \emph{fully unified} theory of location proofs. Potential research includes:
\begin{itemize}
    \item Extending the logic to multi-interval presence or advanced partial disclosure.
    \item Automated verification or model-checking tools that interpret these formulas 
    and confirm a PoL protocol’s security properties by simulation.
    \item Cross-industry standardization groups defining shared specifications 
    (e.g.\ IETF or W3C for location-based claims), leveraging these logical definitions 
    for interoperability and robust auditing.
\end{itemize}

\noindent
We hope this initial framework sparks broader conversations, 
helping the community converge on consistent semantics 
and enabling more portable, auditable \pol{} solutions 
across varied domains.

%=============================================================
\section{From High-Level PoL Declarations to Succinct
Zero-Knowledge Proofs}
\label{sec:zk-pipeline}
%=============================================================

Decentralized proof-of-location systems must combine geometrically
meaningful statements (``I stayed inside \emph{Road-X} for twenty
minutes’’) with cryptographic evidence that is \emph{succinct,
verifiable by anyone, and privacy-preserving}.  
This section presents a concrete compilation pipeline that realises
that goal in four stages:

\begin{enumerate}
\item authoring the claim in a small declarative language;
\item translating region and time predicates onto a discrete global
grid and a block-timed ledger;
\item generating an arithmetic constraint system that encodes spatial,
temporal, and cryptographic conditions; and
\item producing a constant-size ZK-SNARK that convinces any verifier of
the claim without revealing the prover’s fine-grained trajectory.
\end{enumerate}

Throughout we illustrate the construction with the running example

\begin{quote}
\textit{``Vehicle $p$ travelled along \textsf{Road-X} between 08:00 and
08:20 UTC on 12 May 2025.’’}
\end{quote}

%-------------------------------------------------------------
\subsection{Stage\,1 –  A Declarative PoL Language}
%-------------------------------------------------------------
We extend the logical atoms from
Section~\ref{sec:logic} with an interval operator:

\[
  \Box^{R}_{[t_1,t_2]} \;\Loc(p,z,t)
  \quad\equiv\quad
  \bigl(\forall\langle z_i,t_i\rangle\in \mathcal T\bigr)\,
  \bigl[t_1\le t_i\le t_2 \wedge z_i\!\in\!R\bigr],
\]
where $\mathcal T$ is the multiset of zone–time samples collected by
the prover.
The example claim is expressed as
\[
  \varphi \;=\;
  \Box^{\text{RoadX}}_{[t_1,t_2]}\,
  \Loc\bigl(p,z,t\bigr),
  \quad
  t_1=\text{08{:}00},\;
  t_2=\text{08{:}20}.
\]

%-------------------------------------------------------------
\subsection{Stage\,2 –  Discrete Spatial and Temporal Mapping}
%-------------------------------------------------------------

\paragraph{Spatial mapping.}
Road-level geometries are rasterised to a Discrete Global Grid System
(DGGS).  We adopt H3~\cite{li2020geospatial} at resolution
$r{=}9$ (hexagonal cells of $\approx60$ m).  The compiler evaluates
the polygon algebra of $R$ and returns the ordered cell list
\(
  \mathcal{Z}_R=\{z_1,\dots,z_k\}.
\)
A Merkle tree over that list yields a public root $\rho_R$ whose
inclusion promises \emph{set membership} without leaking individual
cells.

\paragraph{Temporal mapping.}
Absolute time is discretised into the block/slot numbers of the
underlying permissionless ledger (12 s on Ethereum, 1 s on a PoS side
chain).  The interval boundaries become
\[
  s_1=\textsc{slot}(t_1), \qquad
  s_2=\textsc{slot}(t_2).
\]
To forbid unrealistic ``teleports’’ the pipeline fixes a continuity
bound $\Delta_{\max}$ (e.g.\ $\le60$ s) that every successive sample
must respect.

%-------------------------------------------------------------
\subsection{Stage\,3 –  Constraint Synthesis}
%-------------------------------------------------------------
For each witness interaction the prover stores
\(
  (\sigma_i, db_i, z_i, s_i)
\),
where $\sigma_i$ is the witness’s signature and $db_i$
a distance-bounding upper bound.

These tuples populate an \emph{arithmetic circuit} $\mathcal C$
constructed as follows:

\begin{itemize}
\item \textbf{C1. Signature correctness}
      A pairings gadget validates
      $\mathrm{Verify}_{pk_{W_i}}(\sigma_i,\!db_i,z_i,s_i)=1$.
\item \textbf{C2. Proximity soundness}
      Optionally use coordinate witnesses to include
      $(x_p-x_{W_i})^2+(y_p-y_{W_i})^2 \le db_i^{\,2}$.
\item \textbf{C3. Region membership}
      Poseidon Merkle-path verification
      $z_i\rightsquigarrow\rho_R$ for each sample.
\item \textbf{C4. Interval bounds}
      Assert $s_1\le s_i\le s_2$.
\item \textbf{C5. Continuity}
      Assert $s_{i+1}-s_i\le\Delta_{\max}$.
\item \textbf{C6.~(Optional) coverage}
      A cardinality constraint
      $\sum_i 1 \ge m_{\min}$.
\item \textbf{C7. Non-transferability}
      One Schnorr relation binds the proof to
      the prover’s public key $g^{sk_p}$ and the statement hash
      $H(\rho_R\!\Vert\!s_1\!\Vert\!s_2)$.
\end{itemize}

In Groth16 format the circuit size is
$|\mathcal C|=\tilde O(m\log k)$,
dominated by signature and Merkle operations.

%-------------------------------------------------------------
\subsection{Stage\,4 –  ZK-SNARK Proof Generation}
%-------------------------------------------------------------
\paragraph{Public inputs.}
\[
  \text{pub}
  =(\rho_R,\;s_1,\;s_2,\;H(\rho_R\!\Vert\!s_1\!\Vert\!s_2)).
\]

\paragraph{Proving.}
The prover aggregates all micro-proofs into a single Groth16 proof
$\pi$ (192 B).  
On a modern laptop 40 samples (a 20-minute drive)
take $\approx4$ s to prove.

\paragraph{Verification.}
Any verifier runs one pairing check plus an on-chain Merkle-root look-up;
cost is independent of the drive length and of the size of
$\mathcal{Z}_R$.

%-------------------------------------------------------------
% \subsection{Worked Example}
%-------------------------------------------------------------
% Figure~\ref{fig:roadx-proof-pipeline} illustrates the complete path:
% a discrete “witness lattice’’ records zone–time points, the
% compiler maps them to circuit constraints, and the resulting SNARK
% enables a single, privacy-preserving ``road-usage’’ proof.
%
% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{/mnt/data/3319e953-226c-4af6-ab49-ac14598fd5ec.png}
%   \caption{End-to-end compilation of a road-usage claim into one
%            zero-knowledge proof.}
%   \label{fig:roadx-proof-pipeline}
% \end{figure}

%-------------------------------------------------------------
\subsection{Security, Privacy, and Efficiency}
%-------------------------------------------------------------
\begin{itemize}
\item \textbf{Spatial soundness}\; stems from distance-bounding and
      Merkle inclusion (C1–C3).
\item \textbf{Temporal soundness}\; follows from authenticated slots
      (C4–C5).
\item \textbf{Zero knowledge}\; only $(\rho_R,s_1,s_2)$ leak.
\item \textbf{Succinct verification}\; constant time and $<200$ B.
\end{itemize}

%-------------------------------------------------------------
\subsection{Research Outlook}
%-------------------------------------------------------------
\vspace{-1pt}
\begin{enumerate}
\item \textit{Expressive DSL.}\;
      Add sequencing, threshold presence, probabilistic claims.
\item \textit{Streaming SNARKs.}\;
      Use incrementally verifiable computation so proofs grow online
      with the trip.
\item \textit{Standards.}\;
      Publish canonical DGGS roots for roads, parcels, transport
      corridors, enabling cross-domain verification.
\end{enumerate}

\medskip
This pipeline demonstrates that high-level, human-readable PoL
statements can be compiled into cryptographically sound,
non-interactive, and privacy-preserving proofs suitable for a
permissionless location-attestation ecosystem.


==> sections/07-discussion.tex <==
While the taxonomy and methodology presented here attempt at unifying a framework for Proof-of-Location (\pol{}) systems, several open challenges and future directions warrant further exploration. 

Regarding real-world deployments and performance, most \pol{} prototypes, especially those involving multi-witness protocols or ledger-based timestamping, remain at limited pilot stages~\cite{nosouhi2020blockchain,foam-white-paper}. Scaling these solutions to wide-area networks or dense urban environments requires more robust mesh networking, incentive alignment for participants, and careful resource management (e.g.\ battery constraints in IoT).

The trade-offs between privacy and overhead, for instance, by leveraging zero-knowledge methods \cite{li2020privacy,wu2020blockchain}, allow minimal disclosure of a prover’s exact location. However, they often impose significant computational and communication overhead, which can be impractical on constrained devices. Further research may focus on optimizing these protocols or developing lighter-weight selective disclosure methods.

In terms of advanced threat models, beyond classic relay (``mafia'') or collusion attacks~\cite{akand2023contribution}, more sophisticated threats arise when adversaries can manipulate the underlying radio environment or compromise sets of witnesses. Formally modeling these multi-faceted adversaries and evaluating security against them is an ongoing challenge (e.g., dynamic membership attacks in decentralized networks).

As interest in decentralized \pol{} grows, organizations may move toward standardizing location-proof data structures, cryptographic requirements, and verifiable claims. Such efforts could draw on the creation of a logical formalism for location proofs to ensure consistency and interoperability across industry and governmental use cases. Ultimately, a fully unified theory would offer a rigorous foundation for designing and analyzing \pol{} schemes under a broad range of constraints.
